Knowledge Distillation for Multi-task Learning

Multi-task learning (MTL) is to learn one single model that performs multiple tasks for achieving good performance on all tasks and lower cost on computation. Learning such a model requires to jointly optimize losses of a set of tasks with different difficulty levels, magnitudes, and characteristics (e.g. cross-entropy, Euclidean loss), leading to the imbalance problem in multi-task learning. To address the imbalance problem, we propose a knowledge distillation based method in this work. We first learn a task-specific model for each task. We then learn the multi-task model for minimizing task-specific loss and for producing the same feature with task-specific models. As the task-specific network encodes different features, we introduce small task-specific adaptors to project multi-task features to the task-specific features. In this way, the adaptors align the task-specific feature and the multi-task feature, which enables a balanced parameter sharing across tasks. Extensive experimental results demonstrate that our method can optimize a multi-task learning model in a more balanced way and achieve better overall performance.

==> Learning to Balance/conclusion.tex <==
% !TEX root = main.tex

In this work, we proposed a knowledge distillation based multi-task method that learns to produce the same features with the single-task networks to address the unbalanced multi-task learning problem with the hypothesis that the solution of the multi-task network should be close to the single task ones' and lie in the intersection of the single solutions. We demonstrated that our method achieves significant performance gains over the state-of-the-art methods, on challenging benchmarks for image classification and scene understanding (semantic segmentation, depth estimation, and surface normal estimation). As future work, we plan to extend our method to multi-task network architecture searching.


==> Learning to Balance/experiments.tex <==
% !TEX root = main.tex


\subsection{Datasets}
We evaluate our method on three multi-task computer vision benchmarks, including SVHN \& Omniglot, NYU-v2, and Cityscapes.\footnote{The implementation of our method is available at \url{https://github.com/VICO-UoE/KD4MTL}.}
% \url{https://anonymous.4open.science/r/KL-MTL/}}

% \noindent \textbf{SVHN \& Omniglot}
\vspace{0.1cm}
\paragraph{SVHN \& Omniglot} consists of two datasets, \ie SVHN~\cite{netzer2011reading} and Omniglot~\cite{lake2015human} where SVHN is a dataset for digital number classification and Omniglot is the one for characters classification. Specifically, SVHN contains 47,217 training images and 26,040 validation images of 10 classes. Omniglot consists of 19,476 training and 6492 validation samples of 1623 categories. As the testing labels are not provided, we evaluate all methods on the validation images and report the accuracy of both tasks. Note that in contrast to the NYU-V2 and Cityscapes datasets where each image is associated with multiple labels, each image in this benchmark is labeled only for one task. Thus the goal is to learn a multi-task network that can learn both tasks from SVHN and Omniglot.

\vspace{0.1cm}
\paragraph{NYU-V2 \cite{silberman2012indoor}} contains RGB-D indoor scene images, where we evaluate performances on 3 tasks, including 13-class semantic segmentation, depth estimation, and surface normals estimation. We use the true depth data recorded by the Microsoft Kinect and surface normals provided in \cite{eigen2015predicting} for depth estimation and surface normal estimation. All images are resized to $288 \times 384$ resolution as \cite{liu2019end}.

\vspace{0.1cm}
\paragraph{Cityscapes \cite{cordts2016cityscapes}} consists of street-view images, each labeled for two tasks: 7-class semantic segmentation\footnote{The original version of Cityscapes provides labels 19-class semantic segmentation. We follow the evaluation protocol in \cite{liu2019end}, we use labels of 7-class semantic segmentation. Please refer to \cite{liu2019end} for more details.} and depth estimation. We resize the images to $128 \times 256$ to speed up the training.

\subsection{Baselines}
In this work, we use the hard parameters sharing architecture for all methods where the early layers of the network are shared across all tasks and the last layers are task-specific (See \Cref{fig:diagram}). We compare our method with two baselines:
\begin{itemize}
	\item \textbf{STL} learns a task-specific model for each task.
	\item \textbf{Uniform}: This vanilla MTL model is trained by minimizing the uniformly weighted loss \Cref{eq:multitask}.
\end{itemize}

We also compare our method to the state-of-the-art MTL methods which are proposed for solving the unbalanced MTL, including Uncert~\cite{kendall2018multi}, MGDA~\cite{sener2018multi}, GradNorm~\cite{chen2017gradnorm} and a knowledge distillation based method, namely BAM~\cite{clark2019bam}, that applies knowledge distillation to network's prediction. On NYU-v2 and Cityscapes, we also compare our method with Gradient Surgery (GS)~\cite{yu2020gradient} and Dynamic Weight Average (DWA) \cite{liu2019end} with using different architectures, \ie SegNet \cite{badrinarayanan2017segnet} and MTAN~\cite{liu2019end} which is the extension of SegNet by introducing task-specific attention modules for each task.


\subsection{Comparison to the State-of-the-art}

\paragraph{Results on SVHN \& Omniglot.}

\begin{figure}
	\centering
	% include first image
	\includegraphics[width=.65\linewidth]{./figures/LeNet.pdf}  
	% \vspace{-.2cm}
	\caption{Network architecture used in SVHN \& Omniglot.}
	\label{fig:LeNet}
	\vspace{-.1cm}
\end{figure}
First, we evaluate all methods on SVHN \& Omniglot. We extend the LeNet to MTL setting (See \Cref{fig:LeNet}) and use the extended network for all methods. We set the batch size of the mini-batch as 512 where 256 samples from SVHN and 256 images from Omniglot. We use Adam \cite{kingma2014adam} for optimizing the networks and adaptors. The learning rate of all task-specific adaptors is 0.01. We train all methods for 300 epochs in total where we scaled the learning rate by 0.85 every 15 epochs. In our method, weights of task-specific losses (\ie $w$ in \Cref{eq:KDMT}) are set uniformly. As a validation set for hyperparameter search ($\lambda$), we randomly pick 10\% of training data. After the best hyperparameters are chosen, we retrain with the full training set and report the median validation accuracy of the last 20 epochs in \Cref{tab:svhnomni}. We search over the set $\lambda=\{1,5,10,20\}$ of $\lambda$ and we chose $\lambda=10$.
% We use Adam for optimizing the network and we report the median validation accuracy of the last 20 epochs in \Cref{tab:svhnomni}. 

\begin{table}[ht]
	\centering
	
% 	\resizebox{15cm}{}
    % \resizebox{\textwidth}{15cm}{!}
    \resizebox{0.5\textwidth}{!}
	{
		\begin{tabular}{ccccc}
			
			
		%  \#label   &  &  & 100 &  & & & & 300 & & \\
		%  \midrule

		\toprule
		Type & Methods & SVHN & Omniglot & avg \\
		\midrule
		\multirow{1}{*}{STL} & -\ - & 88.84 & 65.76 & -\ -\\
		 % & {\bf Ours} & {\bf 88.85} & {\bf 68.15} & -\ -   \\
		\midrule
		\multirow{5}{*}{MTL} & Uniform & 85.88 & 66.91 & 76.40   \\
		% BAM \cite{clark2019bam} & 86.57 & 66.08 & 76.33 \\
		& Uncert \cite{kendall2018multi} & 85.43 & 64.1 & 74.77 \\
		& MGDA \cite{sener2018multi} & 83.93 & 66.8 & 75.37 \\
		& GradNorm \cite{chen2017gradnorm} & 84.48 & 65.55 & 75.02 \\
		& BAM \cite{clark2019bam} & 86.57 & 66.08 & 76.33 \\
		& {\bf Ours} & {\bf 88.05} & {\bf 70.12} & {\bf 79.09}   \\
		% Ours: MTL + l2 + l1  & 87.86 & 69.45 & 78.66 \\
		\bottomrule
		\end{tabular}%
		\vspace{-0.1cm}
		\caption{Testing accuracy on SVHN \& Omniglot.}
		\label{tab:svhnomni}
	}
\end{table}%

\Cref{tab:svhnomni} shows that MTL with uniform loss weights (Uniform) obtains worse results on SVHN while it achieves better performance on Omniglot than STL. The state-of-the-art methods which dynamically weigh the task-specific losses cannot achieve a good trade-off between these two tasks. More specifically, Uncert and GradNorm obtain worse overall performance than STL while MGDA improves the performance on Omniglot and obtains worse performance on SVHN. Though BAM obtains better overall performance on both tasks, the improvement is achieved mainly because of more informative information provided by the continuous predictions of the teacher network (task-specific models). The unbalanced problem in MTL when we use BAM is still unsolved as BAM applies knowledge distillation on network predictions, which would have similar problems with the vanilla MTL (Uniform).
In contrast, our approach achieves significantly better performance than any other MTL methods \ie our method obtains 88.05 \% accuracy on SVHN and 70.12 \% accuracy on Omniglot. Compared with STL, our method obtains comparable results on SVHN and significant gains on Omniglot. These results strongly verify that our method is able to alleviate the unbalanced problem in this benchmark and to outperform STL as it enables the MTL model to learn more informative features.



% We explore the structure of the adaptors and the results are reported in \cref{tab:structure}. It seems that adding some non-linearty does not benefit the training.

% \begin{table}[ht]
% 	\centering
	
% % 	\resizebox{15cm}{}
%     % \resizebox{\textwidth}{15cm}{!}
% 	{
% 		\begin{tabular}{cccccc}
			
			
% 		%  \#label   &  &  & 100 &  & & & & 300 & & \\
% 		%  \midrule

% 		\toprule
% 		Methods & SVHN & Omniglot & avg & structure & dimension \\
% 		\midrule
% 		\multirow{6}{*}{Ours} & 88.05 & 70.12 & 79.09 & conv & -\ -   \\
% 		& 86.23	& 64.43	& 75.33 & conv + relu & -\ - \\
% 		& 86.54 & 65.39	& 75.97 & conv + relu + conv & 20 \\
% 		& 86.78	& 65.70	& 76.24 & conv + relu + conv & 25 \\
% 		& 86.05	& 67.94	& 77.00 & conv + relu + conv & 50 \\
% 		& 85.91	& 68.44	& 77.18 & conv + relu + conv & 100 \\
% 		% Ours: MTL + l2 + l1  & 87.86 & 69.45 & 78.66 \\
% 		\bottomrule
% 		\end{tabular}%
% 		\vspace{0.1cm}
% 		\caption{Testing accuracy on SVHN \& Omniglot.}
% 		\label{tab:structure}
% 	}
% \end{table}%

% Another exploration is to give weight on feature: different channels have different weight $\{0,1\}$ and the weight can be estimate by random or from Fisher Information Matrix (FIM). The results are presented in \cref{tab:selectfeat}

% \begin{table}[ht]
% 	\centering
	
% % 	\resizebox{15cm}{}
%     % \resizebox{\textwidth}{15cm}{!}
% 	{
% 		\begin{tabular}{cccccc}
			
			
% 		%  \#label   &  &  & 100 &  & & & & 300 & & \\
% 		%  \midrule

% 		\toprule
% 		Methods & SVHN & Omniglot & avg & ratio & top-k \\
% 		\midrule
% 		\multirow{2}{*}{Random} & 87.45	& 65.49	& 76.47 & 0.5 & -\ -   \\
% 		& 87.37	& 69.73	& 78.55 & 0.7 & -\ - \\
% 		\multirow{2}{*}{FIM}& 86.85	& 65.33	& 76.09 & -\ - & 25 \\
% 		& 85.59	& 65.26	& 75.425  & -\ - & 40 \\
% 		% Ours: MTL + l2 + l1  & 87.86 & 69.45 & 78.66 \\
% 		\bottomrule
% 		\end{tabular}%
% 		\vspace{0.1cm}
% 		\caption{Testing accuracy on SVHN \& Omniglot.}
% 		\label{tab:selectfeat}
% 	}
% \end{table}%

\begin{table}[t]
	\centering
	
% 	\resizebox{15cm}{}
    \resizebox{1.0\textwidth}{!}
    {
		\begin{tabular}{cccccccccccc}
			
			
		  %  \#label   &  &  & 100 &  & & & & 300 & & \\
		  %  \midrule

		    \toprule
		    \multirow{4}{*}{Architecture} & \multirow{4}{*}{Type} & \multirow{4}{*}{Methods} & \multicolumn{2}{c}{Segmentation} & \multicolumn{2}{c}{Depth} & \multicolumn{5}{c}{Surface Normal} \\
		    & & &  \multicolumn{2}{c}{\multirow{2}{*}{(Higher Better $\uparrow$)}}
		     & \multicolumn{2}{c}{\multirow{2}{*}{(Lower Better $\downarrow$)}}
		   & \multicolumn{2}{c}{Angle Distance} & \multicolumn{3}{c}{Within $t^{\circ}$}\\
		     & & & & & & &  \multicolumn{2}{c}{(Lower Better $\downarrow$)} & \multicolumn{3}{c}{(Higher Better $\uparrow$)}\\
		    & & & mIoU & Pix Acc & Abs Err & Rel Err & Mean & Median & 11.25 & 22.5 & 30 \\
		    \midrule
		    \multirow{6}{*}{SegNet} & STL & -\ - & 17.32 & 55.70 & 0.6577 & 0.2828 & 29.99 & 23.81 & 24.31 & 48.06 & 60.05 \\
		    \cmidrule{2-12}
		     & \multirow{5}{*}{MTL} & Uniform & 18.14 & 55.82 & 0.5841 & 0.2490 & 31.89 & 26.81 & 20.61 & 42.95 & 55.33 \\
		     & & Uncert \cite{kendall2018multi} & 16.79 & 52.51 & 0.6183 & 0.2612 & 32.44 & 27.27 & 20.81 & 42.41 & 54.47 \\
			 & & MGDA \cite{sener2018multi} & 15.57 & 49.05 & 0.6716 & 0.2710 & 29.90 & 24.13 & 23.81 & 47.58 & 59.75 \\
			 & & GradNorm \cite{chen2017gradnorm} & 18.08 & 55.76 & 0.5819 & 0.2495 & 30.65 & 25.38 & 22.64 & 45.34 & 57.59 \\
		     % & & MTL + KD \cite{clark2019bam} & 17.00 & 53.34 & 0.6018 & 0.2564 & 32.72 & 27.60 & 20.18 & 41.93 & 53.98 \\
		     % \cmidrule{3-12}
		     & & Ours & {\bf 18.75} & {\bf 58.02} & {\bf 0.5780} & {\bf 0.2467} & {\bf 29.40} & {\bf 23.71} & {\bf 24.33} & {\bf 48.22} & {\bf 60.45}\\
		 	\midrule
		 	
		 	\multirow{8}{*}{MTAN \cite{liu2019end}} & STL & -\ - & 16.38 & 53.89 & 0.6792 & 0.2963 & 30.66 & 24.26 & 23.35 & 47.34  & 59.33 \\
		 	\cmidrule{2-12}
		     & \multirow{7}{*}{MTL} & Uniform & 17.72 & 55.32 & 0.5906 & 0.2577 & 31.44 & 25.37 & 23.17 & 45.65 & 57.48 \\
		     & & DWA \cite{liu2019end} & 17.52 & 55.76 & 0.5869 & 0.2549 & 31.75 & 25.64 & 22.60 & 45.12 & 57.05   \\
		     & & Uncert \cite{kendall2018multi} & 17.67 & 55.61 & 0.5927 & 0.2592 & 31.25 & 25.57 & 22.99 & 45.83 & 57.67 \\
			 & & MGDA \cite{sener2018multi} & 15.60 & 52.36 & 0.6215 & 0.2767 & 30.26 & 24.01 & 23.98 & 47.77 & 59.85 \\
			 & & GradNorm \cite{chen2017gradnorm} & 17.37 & 55.92 & 0.5924 & 0.2630 & 31.20 & 24.91 & 23.11 & 46.27 & 58.20 \\
		     & & GS$^\ast$ \cite{yu2020gradient} & 20.17 & 56.65 & 0.5904 & 0.2467 & 30.01 & 24.83 & 22.28 & 46.12 & 58.77   \\
		    % \midrule
		    % \cmidrule{3-12}
		     & & Ours & {\bf 20.75} & {\bf 57.90} & {\bf 0.5816} & {\bf 0.2445} & {\bf 29.97} & {\bf 23.96} & {\bf 24.24} & {\bf 47.78} & {\bf 59.78} \\
			\bottomrule
		\end{tabular}%
			}
		\vspace{-0.25cm}
		\caption{Testing results on NYU-v2. $^\ast$ Results of the `GS' method are from \cite{yu2020gradient}.}
		\label{tab:nyuv2}
\end{table}%

% \vspace{0.1cm}
\paragraph{Results on NYU-V2.}
% On NYU-V2, we adopt two networks as the based network for all methods, \ie SegNet \cite{badrinarayanan2017segnet} and MTAN \cite{liu2019end} which is the extension of SegNet by introducing task-specific attention modules for each task. 
We follow the training and evaluation protocol in \cite{liu2019end}. We use cross-entropy loss for semantic segmentation, l1-norm loss for depth estimation, and cosine similarity loss for surface normal estimation. We train all methods using Adam \cite{kingma2014adam} with the learning rate initialized at 1e-4 and halved at the 100-th epoch for 200 epochs in total. The learning rate of all task-specific adaptors is 0.1 and the batch size is 2. In our method, weights of task-specific losses (\ie $w$ in \Cref{eq:KDMT}) are set uniformly. As a validation set for hyperparameter search ($\lambda$), we randomly pick 10\% of training data. After the best hyperparameters are chosen, we retrain with the full training set and report the results of three tasks on the validation set in \Cref{tab:nyuv2}. We search over the set $\lambda=\{1,2,3,4,5,6\}$ of $\lambda$ and the distillation loss' weight of Segmentation, depth, and surface normal are set to 1, 1 and 2, respectively.
% $\lambda$ in \cref{eq:KDMT} is 2. 
% As a validation set for hyperparameter search ($\lambda$), we randomly pick 10\% of training data. After the best hyperparameters are chosen, we retrain with the full training set and report the median validation accuracy of the last 20 epochs in \Cref{tab:svhnomni}. We search over the set $\lambda=\{1,5,10,20\}$ of $\lambda$ and we chose $\lambda=10$.

% We set the batch size as 2 and report the results of three tasks in \cref{tab:nyuv2}.



% The results are shown in \cref{tab:nyuv2}. 


% \begin{table}[ht]
% 	\centering
	
% % 	\resizebox{15cm}{}
%     \resizebox{1.0\textwidth}{!}
%     {
% 		\begin{tabular}{ccccccccccc}
			
			
% 		  %  \#label   &  &  & 100 &  & & & & 300 & & \\
% 		  %  \midrule

% 		    \toprule
% 		    \multirow{4}{*}{Backbone} & \multirow{4}{*}{Methods} & \multicolumn{2}{c}{Segmentation} & \multicolumn{2}{c}{Depth} & \multicolumn{5}{c}{Surface Normal} \\
% 		    & &  \multicolumn{2}{c}{\multirow{2}{*}{(Higher Better $\uparrow$)}}
% 		     & \multicolumn{2}{c}{\multirow{2}{*}{(Lower Better $\downarrow$)}}
% 		   & \multicolumn{2}{c}{Angle Distance} & \multicolumn{3}{c}{Within $t^{\circ}$}\\
% 		     & & & & & &  \multicolumn{2}{c}{(Lower Better $\downarrow$)} & \multicolumn{3}{c}{(Higher Better $\uparrow$)}\\
% 		    & & mIoU & Pix Acc & Abs Err & Rel Err & Mean & Median & 11.25 & 22.5 & 30 \\
% 		    \midrule
% 		    \multirow{4}{*}{SegNet} & STL & 17.32 & 55.70 & 0.6577 & 0.2828 & 29.99 & 23.81 & 24.31 & 48.06 & 60.05 \\
% 		     & MTL & 18.14 & 55.82 & 0.5841 & 0.2490 & 31.89 & 26.81 & 20.61 & 42.95 & 55.33 \\
% 		     & MTL + KD \cite{clark2019bam} & 17.00 & 53.34 & 0.6018 & 0.2564 & 32.72 & 27.60 & 20.18 & 41.93 & 53.98 \\
% 		     & Ours & {\bf 18.75} & {\bf 58.02} & {\bf 0.5780} & {\bf 0.2467} & {\bf 29.40} & {\bf 23.71} & {\bf 24.33} & {\bf 48.22} & {\bf 60.45}\\
% 		 	\midrule
		 	
% 		 	\multirow{4}{*}{MTAN \cite{liu2019end}} & STL & 16.38 & 53.89 & 0.6792 & 0.2963 & 30.66 & 24.26 & 23.35 & 47.34  & 59.33 \\
% 		     & MTL \cite{liu2019end} & 17.52 & 55.76 & 0.5869 & 0.2549 & 31.75 & 25.64 & 22.60 & 45.12 & 57.05   \\
% 		     & Gradient Surgery \cite{yu2020gradient} & 20.17 & 56.65 & 0.5904 & 0.2467 & 30.01 & 24.83 & 22.28 & 46.12 & 58.77   \\
% 		    % \midrule
% 		     & Ours & {\bf 20.75} & {\bf 57.90} & {\bf 0.5816} & {\bf 0.2445} & {\bf 29.97} & {\bf 23.96} & {\bf 24.24} & {\bf 47.78} & {\bf 59.78} \\
% 			\bottomrule
% 		\end{tabular}%
% 			}
% 		\vspace{0.1cm}
% 		\caption{Testing results on NYU-v2.}
% 		\label{tab:nyuv2}
% \end{table}%



% \hb{This is the longest paragraph that I have ever seen in a paper!}
From the results shown in \Cref{tab:nyuv2}, we can see that it is possible to tackle multiple tasks within a network and achieve performance improvement on some tasks, \eg when we use SegNet as the based network, the vanilla MTL (Uniform) achieves better performance on semantic segmentation and depth estimation though it causes a drop on surface normal estimation in comparison with STL. Though we see the benefits of using MTL, it is also clear that the unbalanced problem exists. 
% On NYU-V2, we jointly optimize multiple losses and we use a task-specific loss function for each task, \ie we use cross-entropy loss for semantic segmentation, l1-norm loss for depth estimation and cosine similarity loss for surface normal estimation). 
% This results in the unbalanced problem as different tasks' losses are quite different and the task with much larger loss may dominate the training, which is also verified in \cite{kendall2018multi,sener2018multi}. 
We then apply existing methods that introduce loss weighting strategies for addressing the unbalanced loss optimization problem. From the results of using SegNet, GradNorm performs the best among all compared methods. However, it provides limited control on the learned parameters (\eg it achieves similar results to the MTL model using a uniformly weighting scheme) and still suffers from lower task performance than the single task models.

In comparison with these methods, our method obtains significant gains over all tasks and achieves better results than single task learning models. This strongly verifies our hypothesis that the solution of the multi-task network should be close to the single task ones' and lie in the intersection of the single-task solutions
 % (illustrated in \cref{fig:learning}) 
and our method that applies stricter control on the parameters of the multi-task network can better address the unbalanced loss problem.

% The results again indicate that our method is able to optimize the MTL model in a more balance way and achieves overall improvement. From another perspective, as illustrated in \cref{fig:learning}, in MTL, jointly optimizing multiple task-specific loss may lead to the unbalanced problem where the MTL model bias to the low error area of one task as one task's gradient may dominate. However, our method assists the MTL model to find the intersection of the low error area of all tasks, which also alleviate the unbalanced problem in MTL. In addition, our method enables the MTL model to learn more informative features for all tasks and the task-specific adaptors loosen the distillation loss, allowing our method to outperform single task learning.



\begin{table}[t]
	\centering
	
% 	\resizebox{15cm}{}
    \resizebox{.7\textwidth}{!}
    {
		\begin{tabular}{ccccccc}
			
			
		  %  \#label   &  &  & 100 &  & & & & 300 & & \\
		  %  \midrule

		    \toprule
		    \multirow{3}{*}{Architecture} & \multirow{3}{*}{Type} & \multirow{3}{*}{Methods} & \multicolumn{2}{c}{Segmentation} & \multicolumn{2}{c}{Depth} \\
		    & & &  \multicolumn{2}{c}{{(Higher Better $\uparrow$)}}
		     & \multicolumn{2}{c}{{(Lower Better $\downarrow$)}}\\
		    & & & mIoU & Pix Acc & Abs Err & Rel Err\\
		    \midrule
		    \multirow{7}{*}{SegNet} & STL & -\ - & 51.85 & 91.08 & 0.0136 & 22.68   \\
		    \cmidrule{2-7}
		     & \multirow{5}{*}{MTL} & Uniform & 50.73 & 90.76 & 0.0151 & 40.81\\
		     & & Uncert \cite{kendall2018multi} & 51.09 & 90.85 & 0.0143 & 27.66 \\
			 & & MGDA \cite{sener2018multi} & 51.69 & 90.99 & {\bf 0.0130} & {\bf 24.04} \\
			 & & GradNorm \cite{chen2017gradnorm} & 50.06 & 90.82 & 0.0143 & 28.61 \\
			 & & Ours & {\bf 52.18} & {\bf 91.24} & 0.0140 & 28.90 \\
		     % & & Ours (last layer) &  52.00 & 91.08 & 0.0147 & 29.25\\
		     % & & Ours (mid+last layer) & 51.99 & 91.04 & 0.0147 & 30.29 \\
		    \midrule
		    \multirow{8}{*}{MTAN} & STL & -\ - & 51.24 & 91.16 & 0.0137 & 24.80   \\
		    \cmidrule{2-7}
		     & \multirow{6}{*}{MTL} & Uniform & 52.56 & 91.33 & 0.0152 & 24.64 \\
		     & & DWA \cite{liu2019end} & 51.95 & 91.33 & 0.0141 & 30.03 \\
		     & & Uncert \cite{kendall2018multi} & 50.37 & 91.11 & 0.0142 & 31.78 \\
			 & & MGDA \cite{sener2018multi} & 52.32 & {\bf 91.59} & {\bf 0.0138} & 30.35 \\
			 & & GradNorm \cite{chen2017gradnorm} & 51.88 & 91.40 & 0.0148 & 31.43 \\
			 & & Ours & {\bf 52.71} & 91.54 & 0.0139 & {\bf 27.33} \\
		  %    &  & Ours (last layer) & 52.47 & 91.32 & 0.0143 & 27.95 \\
			 % & & Ours (mid+last layer) & 52.49 & 91.40 & 0.0148 & 28.44 \\
		     \bottomrule
		\end{tabular}%
		}
		\vspace{-0.3cm}
		\caption{Testing results on Cityscapes.}
		\label{tab:cityscapes}
\end{table}%



% \vspace{0.1cm}
\paragraph{Results on Cityscapes.}
Similar to NYU-V2, we use cross-entropy loss for semantic segmentation and l1-norm loss for depth estimation in Cityscapes as in \cite{liu2019end}.
% we also evaluate all methods on the Cityscapes using two based network, the SegNet \cite{badrinarayanan2017segnet} and MTAN \cite{liu2019end}. We follow the training and evaluation protocol in \cite{liu2019end}. 
We train all methods using Adam \cite{kingma2014adam} with the learning rate initialized at 1e-4 and halved at the 100-th epoch for 200 epochs in total. The learning rate of all task-specific adaptors is 0.1 and the batch size is 8. In our method, weights of task-specific losses (\ie $w$ in \Cref{eq:KDMT}) are set uniformly.
As a validation set for hyperparameter search ($\lambda$), we randomly pick 10\% of training data. After the best hyperparameters are chosen, we retrain with the full training set and report the results of two tasks on the validation set in \Cref{tab:cityscapes}. We search over the set $\lambda=\{1,2,3,4,5,6\}$ of $\lambda$ and the distillation loss' weight of Segmentation and depth are set to 2 and 6, respectively.




As shown in \Cref{tab:cityscapes}, in overall, MTL obtains worse performance than STL. It is clear that GradNorm obtains worse performance on semantic segmentation while it improves the performance on depth estimation. However, MGDA assigns much larger weight on depth estimation task and this enables the MTL model to achieve better performance on both tasks. Our method also achieves significant gains on both tasks. The results again demonstrate that our method is able to optimize MTL model in a more balanced way and to achieve better overall results.


% \subsection{Compared with Related Knowledge Distillation Methods}

% \begin{table}[ht]
% 	\centering
	
% % 	\resizebox{15cm}{}
%     % \resizebox{\textwidth}{15cm}{!}
% 	{
% 		\begin{tabular}{cccc}
			
			
% 		%  \#label   &  &  & 100 &  & & & & 300 & & \\
% 		%  \midrule

% 		\toprule
% 		 Methods & SVHN & Omniglot & avg \\
% 		\midrule
% 		BAM \cite{clark2019bam} & 86.57 & 66.08 & 76.33 \\
% 		AT \cite{zagoruyko2016paying} & \\
% 		{\bf Ours} & {\bf 88.05} & {\bf 70.12} & {\bf 79.09}   \\
% 		% Ours: MTL + l2 + l1  & 87.86 & 69.45 & 78.66 \\
% 		\bottomrule
% 		\end{tabular}%
% 		\vspace{0.1cm}
% 		\caption{Testing accuracy on SVHN \& Omniglot.}
% 		\label{tab:svhnomniKD}
% 	}
% \end{table}%

% \begin{table}[ht]
% 	\centering
	
% % 	\resizebox{15cm}{}
%     \resizebox{1.0\textwidth}{!}
%     {
% 		\begin{tabular}{ccccccccccc}
			
			
% 		  %  \#label   &  &  & 100 &  & & & & 300 & & \\
% 		  %  \midrule

% 		    \toprule
% 		    \multirow{4}{*}{Architecture} & \multirow{4}{*}{Methods} & \multicolumn{2}{c}{Segmentation} & \multicolumn{2}{c}{Depth} & \multicolumn{5}{c}{Surface Normal} \\
% 		    & &  \multicolumn{2}{c}{\multirow{2}{*}{(Higher Better $\uparrow$)}}
% 		     & \multicolumn{2}{c}{\multirow{2}{*}{(Lower Better $\downarrow$)}}
% 		   & \multicolumn{2}{c}{Angle Distance} & \multicolumn{3}{c}{Within $t^{\circ}$}\\
% 		     & & & & & &  \multicolumn{2}{c}{(Lower Better $\downarrow$)} & \multicolumn{3}{c}{(Higher Better $\uparrow$)}\\
% 		    & & mIoU & Pix Acc & Abs Err & Rel Err & Mean & Median & 11.25 & 22.5 & 30 \\
% 		    \midrule
% 		    \multirow{3}{*}{SegNet} & BAM \cite{clark2019bam} & 17.00 & 53.34 & 0.6018 & 0.2564 & 32.72 & 27.60 & 20.18 & 41.93 & 53.98 \\
% 		    & AT & \\
% 		     % \cmidrule{3-12}
% 		     & Ours & {\bf 18.75} & {\bf 58.02} & {\bf 0.5780} & {\bf 0.2467} & {\bf 29.40} & {\bf 23.71} & {\bf 24.33} & {\bf 48.22} & {\bf 60.45}\\
% 		 	\midrule
		 	
% 		 	\multirow{3}{*}{MTAN \cite{liu2019end}} & BAM & \\
% 		 	& AT & \\
% 		     & Ours & {\bf 20.75} & {\bf 57.90} & {\bf 0.5816} & {\bf 0.2445} & {\bf 29.97} & {\bf 23.96} & {\bf 24.24} & {\bf 47.78} & {\bf 59.78} \\
% 			\bottomrule
% 		\end{tabular}%
% 			}
% 		\vspace{0.1cm}
% 		\caption{Testing results on NYU-v2.}
% 		\label{tab:nyuv2KD}
% \end{table}%

% \begin{table}[ht]
% 	\centering
	
% % 	\resizebox{15cm}{}
%     \resizebox{1.0\textwidth}{!}
%     {
% 		\begin{tabular}{cccccc}
			
			
% 		  %  \#label   &  &  & 100 &  & & & & 300 & & \\
% 		  %  \midrule

% 		    \toprule
% 		    \multirow{3}{*}{Architecture} & \multirow{3}{*}{Methods} & \multicolumn{2}{c}{Segmentation} & \multicolumn{2}{c}{Depth} \\
% 		    & &  \multicolumn{2}{c}{{(Higher Better $\uparrow$)}}
% 		     & \multicolumn{2}{c}{{(Lower Better $\downarrow$)}}\\
% 		    & & mIoU & Pix Acc & Abs Err & Rel Err\\
% 		    \midrule
% 		    \multirow{4}{*}{SegNet} & BAM & \\
% 		    & AT & \\
% 		     & Ours (last layer) &  52.00 & 91.08 & 0.0147 & 29.25\\
% 		     & Ours (mid+last layer) & 51.99 & 91.04 & 0.0147 & 30.29 \\
% 		    \midrule
% 		    \multirow{4}{*}{MTAN} & BAM & \\
% 		    & AT & \\
% 		    & Ours (last layer) & 52.47 & 91.32 & 0.0143 & 27.95 \\
% 			& Ours (mid+last layer) & 52.49 & 91.40 & 0.0148 & 28.44 \\
% 		     \bottomrule
% 		\end{tabular}%
% 		}
% 		\vspace{0.1cm}
% 		\caption{Testing results on Cityscapes.}
% 		\label{tab:cityscapesKD}
% \end{table}%


\subsection{Ablation Study}

To better analyze the effect of the distillation loss, we conduct an ablation study on NYU-V2. We first evaluate the effect of applying distillation loss to more layer's features. On NYU-V2, we report the results of applying distillation loss to the last shared layer's feature only and the results of applying distillation loss to features of both the middle layer and the last layer. From the results presented in \Cref{tab:ablanyuv2}, adding more layers' features for computing distillation loss boosts the performance on NYU-V2 in general. However, results on SVHN \& Omniglot and Cityscapes indicate that using the last layers obtains the best performance. We argue that adding more layers can enhance the distillation loss and a more strict control on the parameters of the multi-task network. This is not necessary for those tasks that use a small network, \eg the network we used in SVHN \& Omniglot and would be useful for tasks using a large network, \eg the SegNet used in NYU-V2.


% \begin{table}[ht]
% 	\centering
	
% % 	\resizebox{15cm}{}
%     \resizebox{1.0\textwidth}{!}
% 	{
% 		\begin{tabular}{cccccccccccc}
			
			
% 		  %  \#label   &  &  & 100 &  & & & & 300 & & \\
% 		  %  \midrule

% 		    \toprule
% 		    & & \multicolumn{2}{c}{Segmentation} & \multicolumn{2}{c}{Depth} & \multicolumn{5}{c}{Surface Normal} \\
% 		    \multicolumn{2}{c}{Method}&  \multicolumn{2}{c}{\multirow{2}{*}{(Higher Better $\uparrow$)}}
% 		     & \multicolumn{2}{c}{\multirow{2}{*}{(Lower Better $\downarrow$)}}
% 		    & \multicolumn{2}{c}{Angle Distance} & \multicolumn{3}{c}{Within $t^{\circ}$}\\
% 		    &  &  & & & &  \multicolumn{2}{c}{(Lower Better $\downarrow$)} & \multicolumn{3}{c}{(Higher Better $\uparrow$)}\\
% 		    Backbone & \#layers  & mIoU & Pix Acc & Abs Err & Rel Err & Mean & Median & 11.25 & 22.5 & 30 \\
% 		    \midrule
% 		    % \midrule
% 		    \multirow{2}{*}{SegNet} & last & 18.66 & 57.78 & 0.5813 & {\bf 0.2375} & 30.17 & 24.74 & 22.96 & 46.44 & 58.76\\
% 		     % & mid + last & {\bf 19.12} & {\bf 58.04} & 0.5835 & 0.2468 & 29.79 & 24.15 & 23.95 & 47.40 & 59.56\\
% 		     & mid + last & {\bf 18.75} & {\bf 58.02} & {\bf 0.5780} & 0.2467 & {\bf 29.40} & {\bf 23.71} & {\bf 24.33} & {\bf 48.22} & {\bf 60.45}\\
% 		 	\midrule
% 		    % \midrule
% 		    \multirow{2}{*}{MTAN \cite{liu2019end}}  & last  & 18.52 & 56.81 & {\bf 0.5756} & 0.2489 & 31.13 & 24.93 & 23.52 & 46.29 &58.18 \\
% 		     % & mid + last  & 20.57 & {\bf 58.40} & 0.5896 & 0.2483 & 30.13 & 24.40 & 23.72 & 46.99 &59.11 \\
% 		     & mid + last  & {\bf 20.75} & {\bf 57.90} & 0.5816 & {\bf 0.2445} & {\bf 29.97} & {\bf 23.96} & {\bf 24.24} & {\bf 47.78} & {\bf 59.78} \\
% 			\bottomrule
% 		\end{tabular}%
% 		}
% 		\vspace{-0.1cm}
% 		\caption{Ablation study on NYU-v2. Here, `\#layer' means which layers are selected for computing distillation loss.}
% 		\label{tab:ablanyuv2}
% \end{table}%

\begin{table}[t]
	\centering
	
% 	\resizebox{15cm}{}
    \resizebox{1.0\textwidth}{!}
	{
		\begin{tabular}{ccccccccccccc}
			
			
		  %  \#label   &  &  & 100 &  & & & & 300 & & \\
		  %  \midrule

		    \toprule
		    & & & \multicolumn{2}{c}{Segmentation} & \multicolumn{2}{c}{Depth} & \multicolumn{5}{c}{Surface Normal} \\
		    \multicolumn{3}{c}{Method}&  \multicolumn{2}{c}{\multirow{2}{*}{(Higher Better $\uparrow$)}}
		     & \multicolumn{2}{c}{\multirow{2}{*}{(Lower Better $\downarrow$)}}
		    & \multicolumn{2}{c}{Angle Distance} & \multicolumn{3}{c}{Within $t^{\circ}$}\\
		    &  &  & & & & &  \multicolumn{2}{c}{(Lower Better $\downarrow$)} & \multicolumn{3}{c}{(Higher Better $\uparrow$)}\\
		    backbone & \#layers & adaptors  & mIoU & Pix Acc & Abs Err & Rel Err & Mean & Median & 11.25 & 22.5 & 30 \\
		    \midrule
		    % \midrule
		    \multirow{4}{*}{SegNet} & last & linear & 18.66 & 57.78 & 0.5813 & {\bf 0.2375} & 30.17 & 24.74 & 22.96 & 46.44 & 58.76\\
		     % & mid + last & {\bf 19.12} & {\bf 58.04} & 0.5835 & 0.2468 & 29.79 & 24.15 & 23.95 & 47.40 & 59.56\\
		     & mid + last & linear & 18.75 & 58.02 & {\bf 0.5780} & 0.2467 & {\bf 29.40} & {\bf 23.71} & {\bf 24.33} & {\bf 48.22} & {\bf 60.45}\\
		     & mid + last & non-linear & {\bf 19.00} & {\bf 58.12} & 0.5853 & 0.2398 & 29.74 & 24.25 & 23.06 & 47.16 & 59.53\\
		     & mid + last & \xmark & 17.11 & 54.60 & 0.6060 & 0.2586 & 30.32 & 24.74 & 22.66 & 46.36 & 58.72\\
		     % & mid + last & linear & 18.75 & 58.02 & {\bf 0.5780} & 0.2467 & {\bf 29.40} & {\bf 23.71} & {\bf 24.33} & {\bf 48.22} & {\bf 60.45}\\
		 	\midrule
		    % \midrule
		    \multirow{4}{*}{MTAN \cite{liu2019end}}  & last & linear & 18.52 & 56.81 & {\bf 0.5756} & 0.2489 & 31.13 & 24.93 & 23.52 & 46.29 &58.18 \\
		     % & mid + last  & 20.57 & {\bf 58.40} & 0.5896 & 0.2483 & 30.13 & 24.40 & 23.72 & 46.99 &59.11 \\
		     & mid + last & linear & {\bf 20.75} & {\bf 57.90} & 0.5816 & {\bf 0.2445} & {\bf 29.97} & {\bf 23.96} & {\bf 24.24} & {\bf 47.78} & {\bf 59.78} \\
		     & mid + last & non-linear & 20.42 & 56.93 & 0.5975 & 0.2589 & 30.32 & 24.86 & 22.98 & 46.21 & 58.55 \\
		     & mid + last & \xmark & 19.30 & 53.85 & 0.6064 & 0.2567 & 31.43 & 27.61 & 17.61 & 40.86 & 54.63 \\
		     % & mid + last & linear & {\bf 20.75} & {\bf 57.90} & 0.5816 & {\bf 0.2445} & {\bf 29.97} & {\bf 23.96} & {\bf 24.24} & {\bf 47.78} & {\bf 59.78} \\
			\bottomrule
		\end{tabular}%
		}
		\vspace{-0.1cm}
		\caption{Ablation study on NYU-v2. Here, `\#layer' means which layers are selected for computing distillation loss. `adaptors' indicates which kind of adaptors is used and `\xmark' means no adaptors are used.}
		\label{tab:ablanyuv2}
\end{table}%



\paragraph{Analysis on Adaptors.} We evaluate our method using different types of adaptors. As mentioned in \Cref{sec:method}, we use a linear layer that consists of a $1\times1\times C\times C$ convolution for each adaptor and denote as `linear' in \Cref{tab:ablanyuv2}. We also evaluate our method without any adaptors (\ie indicated as `\xmark') and with `non-linear 'adaptors (\ie each adaptors consists of a $1\times 1 \times C \times 2C$ convolution, a Relu activation layer and a $1\times 1 \times 2C \times C$ convolution). From the results shown in \Cref{tab:ablanyuv2}, it is clear to see that the adaptors help to align the features of multi-task and single-task as each single-task model produce different features. Compared with our method using `non-linear' adaptors, which have much larger capacity of mapping features, the results indicate that using `linear' adaptors is sufficient as we discuss in \Cref{sec:method}.




\begin{figure}[t]
	\vspace{-0.2cm}
	\RawFloats
	\centering
	\begin{minipage}[t]{0.44\textwidth}
	\centering
	\includegraphics[width=0.99\linewidth]{./figures/Training-loss-svhn.pdf}
	\vspace{-0.6cm}
	\caption{Task-specific loss and distillation loss on training set of SVHN \& Omniglot. Best view in color.}
	\label{fig:svhn}
	\end{minipage}
	\hspace{0.1cm}
	\begin{minipage}[t]{0.46\textwidth}
	\centering
	\includegraphics[width=0.99\linewidth]{./figures/NYU-v2-Training-loss.pdf}
	\vspace{-0.6cm}
	\caption{Task-specific loss and distillation loss on training set of NYU-V2. Best view in color.}
	\label{fig:nyu} 
	\end{minipage}
	\vspace{-0.4cm}
\end{figure}

\paragraph{Further Analysis.}
We also plot the task-specific loss and distillation loss on the training set of two benchmarks for analyzing our method. In both \Cref{fig:svhn} and \Cref{fig:nyu}, it is clear that distillation loss is more balanced than task-specific loss. More specifically, the task-specific loss of SVHN and Omniglot converge at around 0.137 and 1.492, respectively. In contrast, the distillation loss of SVHN and Omniglot converge at around 0.089 and 0.041, respectively. On NYU-V2, the task-specific loss of semantic segmentation, depth estimation, and surface normal estimation end up at 0.027, 0.127, and 0.039 while the distillation loss ends up at around 0.534, 0.381, and 0.364. These results again verify that our method can optimize the MTL method in a more balanced way. 

% \begin{figure}[h]
% 	\centering
% 	% include first image
% 	\includegraphics[width=.4\linewidth]{./figures/Training-loss-svhn.pdf}  
% 	\vspace{-.2cm}
% 	\caption{Diagram of our proposed method. Best seen in color.}
% 	\label{fig:svhn}
% 	\vspace{-.1cm}
% \end{figure}

% \begin{figure}[h]
% 	\centering
% 	% include first image
% 	\includegraphics[width=.4\linewidth]{./figures/NYU-v2-Training-loss.pdf}  
% 	\vspace{-.2cm}
% 	\caption{Diagram of our proposed method. Best seen in color.}
% 	\label{fig:nyu}
% 	\vspace{-.1cm}
% \end{figure}



==> Learning to Balance/intro.tex <==
% !TEX root = main.tex


The objective of multi-task learning (MTL)~\cite{caruana1997multitask,ruder2017overview} is to develop methods that can tackle a large variety of tasks within a single model.
MTL has multiple practical benefits. 
First, learning shared parameters across multiple tasks leads to representations that can be more data-efficient to train and also generalize better to unseen data.
Second, sharing parameters and computations across tasks can significantly reduce both training and inference time over running multiple individual models, which is especially important in platforms with limited computational resources such as mobile devices.
Therefore there is a growing interest in developing MTL methods and MTL has been successfully applied to machine learning problems in several fields including natural language processing~\cite{clark2019bam}, computer vision~\cite{bilen2016integrated,kokkinos2017ubernet} and speech recognition~\cite{seltzer2013multi}. 

There are at least two challenges to achieve better performance and efficiency with MTL.
The first one is to design a multi-task deep neural network architecture that shares only the relevant parameters across the tasks and keeps the remaining ones task-specific.
This is in contrast to the standard MTL methods that share all the layers except the last few ones across all the tasks.
This heuristic is possibly suboptimal when the tasks have different characteristics and goals (\eg semantically low and high-level tasks), however, searching for an optimal architecture in an exponential configuration space is extremely expensive.
The second one is to develop MTL training algorithms that achieve good performance not only in one of the tasks but in all of them.
This problem is especially important when MTL involves jointly minimizing a set of loss functions for various problems with different difficulty levels, magnitudes, and characteristics (\eg cross-entropy, Euclidean loss). 
Thus a naive strategy of uniformly weighing multiple losses can lead to sub-optimal performances and searching for optimal weights in a continuous hyperparameter space can be prohibitively expensive. 

Concerned with the second problem, previous work \cite{chen2017gradnorm,sener2018multi,kendall2018multi,guo2018dynamic,liu2019end} addresses the \emph{unbalanced loss optimization} problem with balanced loss weighting and parameter updating strategies.
Kendall~\etal~\cite{kendall2018multi} weigh loss functions by considering the task-dependent uncertainty of the model at training time.
Sener~\etal~\cite{sener2018multi} pose the MTL as a multiple objective optimization problem and propose an approximate Pareto optimization method that uses Frank-Wolfe algorithm to solve the constrained optimization.
Yu~\etal~\cite{yu2020gradient} project the gradients for each loss function to a space where conflicting gradient components are removed to eliminate the disturbance between the tasks.
Although the previous work improves over the uniform weighing loss strategy in MTL, they still suffer from the problem of one task dominating the remaining ones and lower task performance than the single task models in standard multi-task benchmarks.
% Despite of these work, the unbalance problem in multi-task learning remains and leads to worse performance for tasks compared with individual task training.

% Though a variety of work has been proposed for exploring on optimizing such multi-task method, the optimization in multi-task learning remains challenging, sometimes resulting in worse overall performance or some tasks dominate during training. This is mainly caused by the unbalance of different tasks' loss function (\eg different scale loss value or distinct tasks learn at different rate). 
% To address the unbalance problem in multi-task learning, Kendall et al. \cite{kendall2018multi} learn to weigh tasks' losses according the model's uncertainty. Sener et al. \cite{sener2018multi} treat the optimization in multi-task learning as the multiple objectives optimization problem and propose an approximation method to quickly assign weight to each task's loss. In contrast, Yu et al. \cite{yu2020gradient} project all tasks' gradients into a space where conflicting gradient conponents are removed. Despite of these work, the unbalance problem in multi-task learning remains and lead to worse performance for tasks compared with individual task training.
% \begin{figure}[t]
% 	\centering
% 	% include first image
% 	\includegraphics[width=.65\linewidth]{./figures/learning.pdf}  
% 	% \vspace{-.2cm}
% 	\caption{Illustration of the multi-task learning for an example two task scenarios. STL and MTL denote single-task and multi-task learning respectively. The colored regions indicate solution spaces with low generalization error for single task networks. Our hypothesis is that a low generalization error solution can be found in the intersection of two single-task models. Best seen in color.}
% 	\label{fig:learning}
% 	% \vspace{-.1cm}
% \end{figure}


\begin{figure}[t]
	\centering
	% include first image
	\includegraphics[width=.99\linewidth]{./figures/diagram.pdf}  
	% \vspace{-.2cm}
	\caption{Diagram of our method. We first train a task-specific model for each task in an offline stage and freeze their parameters (\ie (a), (c)). We then optimize the parameters of the multi-task network for minimizing a sum of task-specific losses and also for producing similar features with the single-task networks (\ie (b)). Best seen in color.}
	% . \hb{Can you indicate feature encoder $\phi$, predictors $\psi$ and use $A$ instead of $\mathcal{A}$?}}
	\label{fig:diagram}
	\vspace{-.1cm}
\end{figure}

In this paper, we approach the unbalanced MTL problem from a different point and propose a knowledge distillation based method inspired from~\cite{romero2014fitnets,hinton2015distilling}.
As weighing the individual loss functions (\eg \cite{kendall2018multi}) or modifying the gradients for the loss functions by simple transformations (\eg \cite{chen2017gradnorm,yu2020gradient}) provide a limited control on the learned parameters and are thus limited to prevent one task dominating the rest, we propose a more strict control on the parameters of the multi-task network.
Given that single-task networks often perform well with sufficient training data, we hypothesize that the solution of the multi-task network should be close to the single task ones' and lie in the intersection of the single-task solutions.
 % (illustrated in \cref{fig:learning}).
To this end, we first train a task-specific model for each task in an offline stage and freeze their parameters; then optimize the parameters of the multi-task network for minimizing a sum of task-specific losses and also for producing similar features with the single-task networks.
As each task-specific network can compute different features, we introduce small task-specific adaptors that map multi-task features to the task-specific one's.
The adaptors align the features of the single-task and multi-task networks, and enables a balanced parameter sharing across multiple tasks.


% Encouraging the multi-task network to match the features of the single-task networks with some flexibility (\ie via the task-specific adapters) enables to the multi-task network to converge to a good solution while preventing the solution to be dominated by only one task.

% As the unbalance problem remains if we apply distillation loss to tasks' predictions, we consider to distill knowledge from task-specific model to multi-task learning model in feature space. 
% More specifically, we introduce small task-specific adaptors to transform the feature from the multi-task model and using the feature distillation technique to ensure that the multi-task model is trained to produce similar features (\ie the transformed features) to the feature of task-specific models. 
% In this way, we are able to applying the same distillation loss function to the normalized features of different tasks, which are transformed by the task-specific adaptors. 
% This provides more balance losses of multiple tasks for optimization than optimizing task-specific losses. From another perspective, as shown in \cref{fig:learning}, the unbalance problem occurs as one task's gradient may dominate the training and this bias the model to one task's low error area. To prevent this, our method is able to encourage the multi-task model to search the optimum for all tasks in the intersection area of all tasks' low error area. In addition, the adaptors introduced in this work assist the multi-task learning model in learning more informative features which allow the multi-task learning model to outperform the single-task learning.
% From another perspective, as shown 
% In this way, the tasks' losses in multi-task learning are more balanced for optimizing as we use the same distillation loss function for all tasks and the features are normalized. We show that this mitigates the unbalance problem in multi-task learning and enables the multi-task model to achieve better overall performance for all tasks.


In the remainder of this paper, we first discuss how our method relates the previous MTL and data distillation methods in \Cref{sec:rel}, formulate our method in \Cref{sec:method}, demonstrate that our method outperforms the state-of-the-art MTL methods in two standard benchmarks in \Cref{sec:exp} and conclude the paper with future remarks in \Cref{sec:conc}.
% In summary, we introduce a knowledge distillation based method for optimizing multi-task learning model in a more balanced way. We introduce small adaptors to transform features from multi-task learning and distill knowledge from task-specific model to multi-task learning model, which provides more balanced losses for optimization and enables the multi-task learning model to learn more informative features for all tasks. Extensive experimental results on three benchmarks strongly verify the efficacy of our method.


% Existing knowledge distillation techniques \cite{clark2019bam} that directly apply restriction on features are too strict for multi-task learning and may also lead to tasks conflicts in features during optimization, the adaptors proposed in this work relax the restriction of feature distillation and thus yield improvement in overall.



% It is costly and unefficient and neglect the inductive bias among task that may help each task.

% One common way to efficiently, use the MTL technique where we train a single model containing shared module to extract features for all tasks. However, this way focuses too much on feature that are shared across tasks and causes loss of task-specific info.

% In this work, we consider performing MTL optimization in another way, where we trained specialized model for each tasks and compress these specialized models into a single MTL model using Knowledge Distillation Technique. Unlike other KD methods that directly performs knowledge transfer by matching intermediate features or predictions, we design to apply adaptors on MTL' features to construct the feature which is then compared with the teacher network. This loosens the regularization between the student and teacher network and allows the network to learn more informative feature for all tasks.

% loss balance -> matching loss is at the same scale -> we treat each tasks minimum equally -> it is eaiser to find the overlapping area of multiple tasks minimum loss landscape
%              -> CE may be at different scale -> cause the unbalance problem as one of task may dominate during training 

==> Learning to Balance/method.tex <==
% !TEX root = main.tex

\subsection{Single-task Learning (STL)}
% \begin{figure}
% 	\centering
% 	% include first image
% 	\includegraphics[width=.99\linewidth]{./figures/diagram.pdf}  
% 	% \vspace{-.2cm}
% 	\caption{Diagram of our proposed method. Best seen in color.}
% 	% . \hb{Can you indicate feature encoder $\phi$, predictors $\psi$ and use $A$ instead of $\mathcal{A}$?}}
% 	\label{fig:diagram}
% 	\vspace{-.1cm}
% \end{figure}


Consider that we are given a dataset $\mathcal{D}$ that contains $N$ training images $\bx^i$ and their labels $\by_1^i,\dots,\by_T^i$ for $T$ tasks (\eg semantic segmentation, depth estimation, surface normals). 
In case of the STL, we wish to learn $T$ convolutional neural networks, one for each task, each maps the input $\bx$ to the target label $\by_\tau$, \ie $f(\bx;\theta^s_\tau,\vartheta^s_\tau)=\by_\tau$ where the superscript $s$ indicates the single-task, $\theta^s_\tau$ and $\vartheta^s_\tau$ are the parameters of the network.
Each single-task network is composed of two parts: i) a feature encoder $\phi(\cdot;\theta^s_\tau)$ that takes in an image and outputs a high-dimensional encoding $\phi(\bx;\theta^s_\tau)\in\mathbb{R}^{C\times H\times W}$ where $C$, $H$, $W$ are the number channels, height and width of the feature map; ii) a predictor $\psi(\cdot;\vartheta^s_\tau)$ that takes in the encoding $\phi(\bx;\theta^s_\tau)$ and predicts the output for the task $\tau$, \ie $\hat{\by}_\tau=\psi(\cdot;\vartheta^s_\tau)\circ\phi(\bx;\theta^s_\tau)$ where $\theta^s_\tau$ and $\vartheta^s_\tau$ denote the parameters of the feature encoder and predictor respectively.
The parameters for the network can be learned for each task independently by optimizing a task-specific loss function $\ell_\tau(\hat{\by},\by)$ (\eg Cross-Entropy loss function for classification) over the training samples that measure the mismatch between the ground-truth label and prediction as following:
\begin{equation}\label{eq:singletask}
	\min_{\theta^s_\tau,\vartheta^s_\tau}\sum_{\bx,\by_{\tau} \in \mathcal{D}}\ell_{\tau}(\psi(\cdot;\vartheta^s_\tau)\circ\phi(\bx;\theta^s_\tau),\by_{\tau}).
\end{equation}

\subsection{Multi-task Learning (MTL)}
In the case of MTL, we would like to learn one network that shares the majority of its parameters across the tasks and solves all the tasks simultaneously.
Similar to STL, the multi-task network can be decomposed into two parts: i) a feature encoder $\phi(\cdot;\theta^m)$ that encodes the input image into a high-dimensional encoding, now its parameters $\theta^m$ are shared across all the tasks; ii) a task-specific predictor $\psi(\cdot;\vartheta^m_\tau)$ for each task that takes in the shared encoding $\phi(\bx;\theta^m)$ and outputs its prediction for task $\tau$, \ie $\psi(\cdot;\vartheta^m_\tau)\circ\phi(\bx;\theta^m)$.
Note that we use superscript $m$ to denote MTL.
The multi-task network can be learned by optimizing a linear combination of task-specific losses:
\begin{equation}\label{eq:multitask}
	\min_{\theta^m,\vartheta^m_1,\dots,\vartheta^m_T}\sum_{\tau=1}^{T}\sum_{\bx,\by_{\tau} \in \mathcal{D}}w_{\tau}\ell_{\tau}(\psi(\cdot;\vartheta^m_\tau)\circ\phi(\bx;\theta^m),\by_{\tau})
\end{equation}
where $w_{\tau}$ is a scaling hyperparameter for task $\tau$ that is used for balancing the loss functions among the tasks.

In contrast to the STL optimization in \Cref{eq:singletask}, optimizing \Cref{eq:multitask} involves a joint learning of all the task-specific and shared parameters which is typically more challenging when the task-specific loss functions $\ell_{\tau}$ have different characteristics such as their magnitude and dynamics (\eg logarithmic, quadratic).
One solution to balance the loss terms is to search for the best scaling hyperparameters $w_\tau$ by a cross-validation which has two shortcomings.
First, the hyperparameter search in a continuous space is computationally expensive, especially when the number of tasks is large, as each validation step requires the training of the model.
Second, even when the optimal hyperparameters can be found, it may be sub-optimal to use the same fixed ones throughout the optimization.

\subsection{Knowledge Distillation for Multi-task Learning}
Motivated by these challenges, the previous work \cite{chen2017gradnorm,kendall2018multi,sener2018multi} propose dynamic weighing strategies that can adjust them at each training iteration.
Here we argue that these hyperparameters provide a limited control on the parameters of the network for preventing the unbalanced MTL and thus we propose a different view on this problem inspired by the knowledge distillation methods~\cite{romero2014fitnets,hinton2015distilling}.

%In particular, we aim at distilling the knowledge of task-specific models that individually learn for each task into a single model, \ie multi-task learning model. However, the imbalance problem remains if we apply distillation loss to tasks' predictions, we consider to distill knowledge from task-specific model to multi-task learning model in feature space

% To this end, we first train a single model $f_{\hat{\vartheta}_{\tau}}$ on each task $\tau$, where $\hat{\vartheta}_{\tau}=\{\vartheta_{s}, \vartheta_{\tau}\}$ and 
To this end, we first train a task-specific model $f(\cdot;\theta^s_\tau,\vartheta^s_\tau)$ for each task $\tau$ by optimizing \Cref{eq:singletask} in an offline stage, freeze their parameters and use only their feature encoders $\phi(\cdot;\theta^s_\tau)$ to regulate the multi-task network at train time by minimizing the distance between the features of task-specific networks and multi-task network for given training samples (see \Cref{fig:diagram}). 
As the outputs of the task-specific encoders can differ significantly and the feature encoder of the multi-task network cannot match all of them simultaneously.
Instead, we project the output of the multi-task feature encoder into each task-specific one via a task-specific adaptor $A_{\tau}:\mathbb{R}^{C\times H\times W}\rightarrow\mathbb{R}^{C\times H\times W}$ where $H$, $W$ and $C$ are the height, width and depth (number of channels) of the features.
In our experiments, we use a linear layer that consists of a $1 \times 1 \times C\times C$ convolution for each adaptor.
These adaptors are jointly learned along the parameters of the multi-task network to align its features with the single-task feature encoders.

\begin{equation}\label{eq:distlossall}
	\mathcal{L}^d=\sum_{\tau=1}^{T}
	\sum_{\bx,\by_\tau \in \mathcal{D}}
			\ell^{d}(A_{\tau}(\phi(\bx;\theta^m)), \phi(\bx;\theta_{\tau}^s))
\end{equation} where $\ell^{d}$ is the Euclidean distance function between the L2 normalized feature maps:
\begin{equation}
	\ell^{d}(\bm{a},\bm{b})=\left\lVert\frac{\bm{a}}{||\bm{a}||_2}-\frac{\bm{b}}{||\bm{b}||_2}\right\lVert_2^2.
\end{equation}

Now we can write the optimization formulation that is employed to learn the multi-task model as a linear combination of  \Cref{eq:multitask} and \Cref{eq:distlossall}:
\begin{equation}\label{eq:KDMT}
	\min_{\theta^m,\vartheta^m_1,\dots,\vartheta^m_T}
	\sum_{\tau=1}^{T}\sum_{\bx,\by_{\tau} \in \mathcal{D}}w_{\tau}\ell_{\tau}(\psi(\cdot;\vartheta^m_\tau)\circ\phi(\bx;\theta^m),\by_{\tau}) + \lambda_\tau \ell^{d}(A_{\tau}(\phi(\bx;\theta^m)), \phi(\bx;\theta_{\tau}^s))
\end{equation} where $\lambda_\tau$ is the task-specific tradeoff hyperparameter.

\paragraph{Discussion.}
Alternatively, the inverse of each adaptor function can be thought as a mapping from each task-specific representation to a shared representation across all the tasks. 
The assumption here is that a large portion of encodings in the task-specific models is common to all the models up to a simple linear transformation.
While the assumption of linear relations between the features of highly non-linear networks may be surprising, such linear relations have also been observed in multi-domain \cite{rebuffi2018efficient} and multi-task problems \cite{stickland2019bert}.


% \begin{equation}\label{eq:KDMT}
% 	\mathcal{L}(\vartheta)=\frac{1}{T}\sum_{\tau=1}^{T}\left(
% 		\frac{\lambda}{N}\sum_{\bx,\by_\tau \in \mathcal{D}}\left(
% 			\ell^{d}(\mathcal{A}_{\tau}(f_{\vartheta_s}(\bx)), f_{{\vartheta^{\tau}_{s}}^{\star}}(\bx))+\frac{1}{N}\sum_{\bx\in \mathcal{D}}\ell_{\tau}(f_{\{\vartheta_{s}, \vartheta_{\tau}\}}(\bx),\by_{\tau}) \right),
% \end{equation}



% obtain the optimal model $f_{{\hat{\vartheta}_{\tau}}^{\star}}$ with parameters $\hat{\vartheta}^{\star}_{\tau}=\{{\vartheta^{\tau}_{s}}^{\star}, \vartheta^{\star}_{\tau}\}$.  We then use the single model $f_{{\hat{\vartheta}_{\tau}}^{\star}}$ to teach the multi-task model $f_{\vartheta}$ by optimizing the following loss:
% \begin{equation}\label{eq:KDMT}
% \mathcal{L}(\vartheta)=\frac{1}{T}\sum_{\tau=1}^{T}\left(\frac{\lambda}{N}\sum_{\bx\in \mathcal{D}}\ell^{m}(\mathcal{A}_{\tau}(f_{\vartheta_s}(\bx)), f_{{\vartheta^{\tau}_{s}}^{\star}}(\bx))+\frac{1}{N}\sum_{\bx\in \mathcal{D}}\ell_{\tau}(f_{\{\vartheta_{s}, \vartheta_{\tau}\}}(\bx),\by_{\tau}) \right),
% \end{equation}
% where the function $\mathcal{A}_{\tau}:\mathbb{R}^{C\times H\times W}\rightarrow\mathbb{R}^{C\times H\times W}$ is a small task-specific adaptor (\ie a $C\times C$ matrix) for task $\tau$ to transform the intermediate feature of the shared module in multi-task model $f_{\vartheta}$. $\ell^{m}(\cdot)$ is the loss function to encourage the multi-task model to produce similar feature with the single model $f_{{\hat{\vartheta}_{\tau}}^{\star}}$ of task $\tau$ by:
% \begin{equation}
% \ell^{d}(\mathcal{A}_{\tau}(f_{\vartheta_s}(\bx)), f_{{\vartheta^{\tau}_{s}}^{\star}}(\bx))=\left\lVert\frac{\mathcal{A}_{\tau}(f_{\vartheta_s}(\bx))}{||\mathcal{A}_{\tau}(f_{\vartheta_s}(\bx))||_2}-\frac{f_{{\vartheta^{\tau}_{s}}^{\star}}(\bx)}{||f_{{\vartheta^{\tau}_{s}}^{\star}}(\bx)||_2}\right\lVert_2^2.
% \end{equation}




==> Learning to Balance/old_method.tex <==
% !TEX root = main.tex
\subsection{Multi-task Learning}
Consider a dataset that contains $T$ tasks, where task $\tau$ contains $N_{\tau}$ training samples $D_{\tau}\{(\bx_{\tau}^{1}, \by_{\tau}^{1}), \cdots, (\bx_{\tau}^{N_{\tau}}, \by_{\tau}^{N_{\tau}})\}$. Further, we let $f_{\theta}$ denote a hard sharing multi-task learning model (a function parameterized for instance, as a deep neural network) with parameters $\theta=\{\theta_{s}, \theta_{1}, \cdots, \theta_{T}\}$, that is trained to predict labels $\by_{\tau}$ of task $\tau$ from given samples $\bx_{\tau}$ as $\by_{\tau}=f_{\theta}(\bx_{\tau})$. Here, $\theta_{s}$ is the parameters shared across tasks and $\theta_{\tau}$ is the task specific parameters for task $\tau$ to predict the label based on the output from $\theta_{s}$. In multi-task learning, one commonly used criterion of learning $f_{\theta}$ is to minimize the following loss:
\begin{equation}\label{eq:multitask}
\mathcal{L}=\frac{1}{T}\sum_{\tau=1}^{T}\frac{1}{N_{\tau}}\sum_{\bx_{\tau}\in D_{\tau}}\ell_{\tau}(f_{\theta}(\bx_{\tau}),\by_{\tau}),
\end{equation}
where $\ell_{\tau}$ is the loss fuction (\eg Cross-Entropy loss function for classification) for task $\tau$.

\begin{figure}[h]
	\centering
	% include first image
	\includegraphics[width=.65\linewidth]{./figures/learning.pdf}  
	\vspace{-.2cm}
	\caption{Illustration of the learning process for both task 1 and task 2 using single task training, multi-task training and our method. Best seen in color.}
	\label{fig:learning}
	\vspace{-.1cm}
\end{figure}

\subsection{Knowledge Distillation for Multi-task Learning}
However, simply optimizing \cref{eq:multitask} may lead to worse overall performance due to the loss (task) imbalance \cite{sener2018multi,kendall2018multi,chen2017gradnorm} where some tasks' losses may dominate during optimization. Instead of developping a weigting scheme to assign dynamic weight to different tasks' losses, we consider optimizing the multi-task learning model using the idea of knowledge distillation. In another word, we aim at compressing the knowledge of the model that individually learns for each specific task into a single model. 

% To this end, we first train a single model $f_{\hat{\theta}_{\tau}}$ on each task $\tau$, where $\hat{\theta}_{\tau}=\{\theta_{s}, \theta_{\tau}\}$ and 
To this end, we first train a single model on each task $\tau$ and obtain the optimal model $f_{{\hat{\theta}_{\tau}}^{\star}}$ with parameters $\hat{\theta}^{\star}_{\tau}=\{{\theta^{\tau}_{s}}^{\star}, \theta^{\star}_{\tau}\}$.  We then use the single model $f_{{\hat{\theta}_{\tau}}^{\star}}$ to teach the multi-task model $f_{\theta}$:
\begin{equation}\label{eq:KDMT}
\mathcal{L}(\theta)=\frac{1}{T}\sum_{\tau=1}^{T}\left(\frac{\lambda}{N_{\tau}}\sum_{\bx_{\tau}\in D_{\tau}}\ell^{m}(\mathcal{A}_{\tau}(f_{\theta_s}(\bx_{\tau})), f_{{\theta^{\tau}_{s}}^{\star}}(\bx_{\tau}))+\frac{1}{N_{\tau}}\sum_{\bx_{\tau}\in D_{\tau}}\ell_{\tau}(f_{\theta}(\bx_{\tau}),\by_{\tau}) \right),
\end{equation}
where the function $\mathcal{A}_{\tau}:\mathbb{R}^{C\times H\times W}\rightarrow\mathbb{R}^{C\times H\times W}$ is a small adaptor for task $\tau$ to transform the intermediate feature (operate on $C$ dimension only) of the shared module in multi-task model $f_{\theta}$. $\ell^{m}()$ is the loss function to teach the multi-task model to produce similar features with the single model $f_{{\hat{\theta}_{\tau}}^{\star}}$ of task $\tau$ by:
\begin{equation}
\ell^{m}(\mathcal{A}_{\tau}(f_{\theta_s}(\bx_{\tau})), f_{{\theta^{\tau}_{s}}^{\star}}(\bx_{\tau}))=\left\lVert\frac{\mathcal{A}_{\tau}(f_{\theta_s}(\bx_{\tau}))}{||\mathcal{A}_{\tau}(f_{\theta_s}(\bx_{\tau}))||_2}-\frac{f_{{\theta^{\tau}_{s}}^{\star}}(\bx_{\tau})}{||f_{{\theta^{\tau}_{s}}^{\star}}(\bx_{\tau})||_2}\right\lVert_2^2.
\end{equation}




==> Learning to Balance/preamble.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{todonotes}
\usepackage{multirow}
\usepackage[ruled,vlined]{algorithm2e}
% \usepackage{ruler}

\usepackage{subfigure}

\usepackage{booktabs}
\usepackage{xspace}
\usepackage{cleveref}
\usepackage{pifont}
\usepackage{floatrow}
% \usepackage{float}
\floatstyle{plaintop}
\restylefloat{table}


\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
% almost no space paragraph
\renewcommand{\paragraph}{%
	\@startsection{paragraph}{4}{\z@}%
	%{1.5ex \@plus 0.5ex \@minus 0.2ex}%
%	{-1em}%
	{0.1em \@plus 0.5ex \@minus 0.2ex}{-1em}%
	{\normalsize\bf}%
}
\makeatother

\newcommand{\hb}[1]{\textcolor{blue}{[Hakan: #1]}}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


\newcommand{\bbm}{\bm{m}}
\newcommand{\bp}{\bm{p}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bx}{\bm{x}}
\newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}

==> Learning to Balance/rel.tex <==
% !TEX root = main.tex

\subsection{Multi-task Learning}


Multi-task learning (MTL) is one of the long-standing problems in machine learning and has been used broadly \cite{caruana1997multitask,rebuffi2017learning,ruder2017overview,du2018adapting,meyerson2018pseudo,meyerson2018pseudo,zhang2014facial,kendall2018multi,misra2016cross,kokkinos2017ubernet}. In computer vision, MTL has been used for image classification \cite{rebuffi2017learning}, facial landmark regression \cite{zhang2014facial}, segmentation and depth estimation \cite{kendall2018multi} and so on. In this work, we specifically focus on tackling the unbalance in the optimization of multi-task networks to achieve good performance not only in a few tasks but in all tasks.

% we consider one of main problem in multi-task learning: the unbalanced problem in jointly minimizing multiple tasks' losses, which is the main reason that causes worse overall performance. 

In recent years, several methods have been proposed for solving the imbalance problem in MTL by either designing loss weighting schemes~\cite{chen2017gradnorm,kendall2018multi,sener2018multi,liu2019end,guo2018dynamic} to weigh each task-specific loss or modifying parameter updates~\cite{yu2020gradient}. Chen~\etal~\cite{chen2017gradnorm} develop a training strategy, namely GradNorm, that looks at the gradient's norm of each task and learns the weight to normalize each task's gradient so as to balance the losses for MTL. In \cite{sener2018multi}, Sener \etal formulate the MTL as a multiple objectives optimization problem and proposed an approximation Pareto optimization method using Frank-Wolfe algorithm to learn weights of losses.
Kendall~\etal~\cite{kendall2018multi} propose to weigh multiple loss functions by considering the homoscedastic uncertainty of each task during training. To design the weighting scheme, Guo \etal~\cite{guo2018dynamic} observe that the imbalances in task difficulty can lead to an unnecessary emphasis on easier tasks, thus neglecting and slowing progress on difficult tasks. Based on the observation, they introduce dynamic task prioritization for MTL, which allows the model to dynamically prioritize difficult tasks during training, where the difficulty is inversely proportional to performance. Rather than weighing the losses, Yu~\etal~\cite{yu2020gradient} propose a form of gradient ``surgery'' that projects each task's gradient onto the normal plane of the gradient of any other task and modifies the gradients for each task so as to minimize negative conflict with other task gradients during the MTL optimization. 

Unlike existing methods, we propose a knowledge distillation based MTL method to solve the unbalanced loss optimization problem from a different angle. To this end, we first train a task-specific model for each task in an offline stage and freeze their parameters. We then train the MTL network for minimizing task-specific loss and also for producing the same features with the task-specific networks. As the task-specific network encodes different features, we introduce small task-specific adaptors to project multi-task features to the task-specific features. In this way, the adaptors align the task-specific feature and the multi-task feature, which enables a balanced parameter sharing across tasks.

% Unlike existing methods, we propose a new mechanism to optimize MTL models so as to address the imbalance problem. To this end, we introduce the idea of knowledge distillation to enable the MTL model to produce similar feature to the feature of each task-specific model. In this way, we are optimize the MTL model in a more balance way as we apply the same loss function on the normalized feature of the shared parameters in MTL model. In addition, this also enable the MTL model to generate informative feature for each task and finally achieve better overall performance.
% MTL (MTL) is one of hot topic in the machine learning field and it has lead to successes in many applications of machine learning, s in many applications of machine learning, from natural language processing and speech recognition to computer vision and drug discovery. In recent years, numerous work have been proposed 
% \paragraph{Optimization for MTL.}
% \begin{itemize}
% 	\item Sener~\etal~\cite{sener2018multi} formulate the MTL as a multiple objectives learning problem and proposed a method to quickly learns the weight to balance multiple tasks' losses during training.
% 	% MTL as multi-objective optimization \cite{sener2018multi} 
% 	\item Chen~\etal~\cite{chen2017gradnorm} develop a training strategy, namely GradNorm, that looks at the gradient's norm of each task and learns the weight to normalize each task's gradient so as to balance the losses for MTL.
% 	\item Kendall~\etal~\cite{kendall2018multi} propose to weighs multiple loss functions by considering the homoscedastic uncertainty of each task.
% 	\item Guo~\etal~\cite{guo2018dynamic} observe that the imbalances in task difficulty can lead to unnecessary emphasis on easier tasks, thus neglecting and slowing progress on difficult tasks. They introduce dynamic task prioritization for MTL, which allows the model to dynamically prioritize difficult tasks during training, where difficulty is inversely proportional to performance. 
% 	\item Yu~\etal~\cite{yu2020gradient} propose a form of gradient surgery that projects each task's gradient onto the normal plane of the gradient of any other task and modify the gradients for each task so as to minimize negative conflict with other task gradients during the MTL optimization.
% \end{itemize}

% \paragraph{Architecture for MTL}
% \begin{itemize}
% 	\item End-to-end MTL with attention \cite{liu2019end} [\href{http://openaccess.thecvf.com/content_CVPR_2019/papers/Liu_End-To-End_Multi-Task_Learning_With_Attention_CVPR_2019_paper.pdf}{pdf}]
% 	\item two papers about learning to allocate filters for MTL
% \end{itemize}

% \paragraph{Auxiliary Tasks Learning.}

% \begin{itemize}
% 	\item Adapting auxiliary losses using gradient similarity \cite{du2018adapting} [\href{https://openreview.net/pdf?id=r1gl7hC5Km}{pdf}]
% 	\item Pseudo-task Augmentation: From Deep Multitask Learning to Intratask Sharing---and Back \cite{meyerson2018pseudo} [\href{https://arxiv.org/pdf/1803.04062.pdf}{pdf}]
% 	\item Self-supervised generalisation with meta auxiliary learning \cite{liu2019self} [\href{https://openreview.net/pdf?id=S1gd7nCcF7}{pdf}]
% 	\item Facial landmark detection by deep MTL \cite{zhang2014facial} [\href{http://home.ie.cuhk.edu.hk/~ccloy/files/eccv_2014_deepfacealign.pdf}{pdf}]
% \end{itemize}


\subsection{Knowledge Distillation}

Our work is also related to knowledge distillation~\cite{hinton2015distilling,romero2014fitnets,tian2019contrastive,ma2019graph,phuong2019towards}.
Hinton~\etal~\cite{hinton2015distilling} show that distilling the knowledge of the whole ensemble of models to a neural network can achieve better performance and avoid an expensive computation. Romero~\etal~\cite{romero2014fitnets} introduce the knowledge distillation to training a small student network to achieve better performance than the teacher network. Apart from the success in single-task learning, knowledge distillation has also been shown to be effective in MTL. Parisotto~\etal~\cite{parisotto2015actor} exploits the use of deep reinforcement learning and model compression techniques to train a single policy network that learns to perform in multiple tasks by using the guidance of several expert teachers. In the contrast, in \cite{clark2019bam}, Clark \etal extends the Born-Again network \cite{furlanello2018born} to MTL setting for NLP. More specifically, they apply the knowledge distillation loss proposed in \cite{hinton2015distilling} on each task's predictions and propose a weight annealing strategy to update the weight of the distillation losses and multiple tasks losses.

Different from these methods, we aim at solving the unbalanced loss optimization problem in MTL. Aligning the predictions from the multi-task network and the task-specific networks would still result in unbalance as the dimension of tasks' predictions is usually different and we need to use different loss functions for matching different tasks' predictions \cite{clark2019bam}, \eg, a kl-divergence loss for classification and l2-norm loss for regression.
% Applying the distillation loss to model's prediction would result in imbalance as the dimension of tasks' predictions is usually different and we need to use differen loss functions for knowledge distillation \cite{clark2019bam}, \eg, kl-divergence loss for classification and l2-norm loss for regression. 
In this work, we first introduce a task-specific adaptor for each task to transform features from the multi-task network and we apply the same loss function to align the transformed multi-task feature and the task-specific networks' features. We train the MTL network for minimizing task-specific loss and for producing the same feature with task-specific networks. This enables the MTL to share the parameters in a balanced way.
% In this way, the transformed feature of tasks are the same dimensional and normalized, the distillation loss are balanced for optimization. In addition, the adaptors assist the MTL model in learning more informative features.
% More specifically, we apply the same distillation loss to the feature of the shared layers which is transformed by task-specific adaptors rather than apply loss functions to the predictions since the dimension of tasks' predictions is usually different and we need to use differen loss functions for knowledge distillation \cite{clark2019bam}.

% \begin{itemize}
% 	\item Distilling the knowledge in a neural network \cite{hinton2015distilling}
% 	\item Fitnets: Hints for thin deep nets \cite{romero2014fitnets}
% 	\item Attention Transfer \cite{zagoruyko2016paying}
% 	\item Contrastive representation distillation \cite{tian2019contrastive}
% 	\item Graph Representation Learning via Multi-task Knowledge Distillation \cite{ma2019graph}
% 	\item Towards understanding knowledge distillation \cite{phuong2019towards}
% 	\item $\cdots$
% \end{itemize}

% \paragraph{Knowledge Distillation for MTL}
% \begin{itemize}
% 	\item Actor-Mimic \cite{parisotto2015actor} exploits the use of deep reinforcement learning and model compression techniques to train a single policy network that learns to perform in multiple tasks by using the guidance of several expert teachers. They apply knowledge distillation loss on normalized Q-value and features.
% 	\item BAM \cite{clark2019bam} simply extends the Born-Again network to MTL setting for NLP. More specifically, they apply the knowledge distillation loss proposed in \cite{hinton2015distilling} on each task's predictions and propose a weight annealing strategy to update the weight of the distillation losses and multiple tasks losses. 
% 	\item Graph Representation Learning via Multi-task Knowledge Distillation \cite{ma2019graph}
% \end{itemize}

% \subsection{Transfer Learning}
% \begin{itemize}
% 	\item Explicit Inductive Bias for Transfer Learning with Convolutional Networks \cite{li2018explicit}. The paper evaluate the effect of L2, L2-SP, L2-SP-Fisher and other regularizers for transfer learning. The authors found that, L2-SP and L2-SP-Fisher can have better ability to transfer knowledge from the source (pretrained) task to target task. However, they also mentioned that, the L2-SP-Fisher using Fisher information to identify which parameters are more important to the source task, performs slightly worse than the L2-SP as L2-SP-Fisher works for life-long learning and the objectives of transfer learning and life-long learning are different.
% 	\item Compared with \cite{li2018explicit}, Pay Attention to Features, Transfer Learn Faster CNNs \cite{wang2020pay} proposed a feature transfer strategy. In the paper, they design a network to identify the importance of the feature (channel) for transfer learning and a network for prunning the network and accelerate the training. They also demonstrate that they method outperforms the method in \cite{li2018explicit}.
% \end{itemize}


% \section{Potential Direction}

% In taskonomy, we have a set of source tasks $\mathcal{S}=\{s_i\}_{i=1}^{N_s}$ and we aim at training a model $\phi$ on $\mathcal{S}$ to achieve good performance on the target task $t$. One thought from \cite{turner2019blockswap} is: we can first pretrain single model on each task of $\mathcal{S}$ individually. We then using the idea of \cite{turner2019blockswap} to compute Fisher Score of each single model, which represent the relation between the source task $s_i$ and the target task $t$. We then can compute the Fisher Score of each set/combination of source tasks and pick the tasks set that achieves the highest Fisher Score. And we perform MTL on the selected tasks set for the target task. Here, perhaps the Fisher Score of each task can used as the weight of loss. Here, we compute the Fisher information to identify, which pretrain parameters are important to the target task and we use this as relations between the source task to the target task.



==> old_method.tex <==
% !TEX root = main.tex
\subsection{Multi-task Learning}
Consider a dataset that contains $T$ tasks, where task $\tau$ contains $N_{\tau}$ training samples $D_{\tau}\{(\bx_{\tau}^{1}, \by_{\tau}^{1}), \cdots, (\bx_{\tau}^{N_{\tau}}, \by_{\tau}^{N_{\tau}})\}$. Further, we let $f_{\theta}$ denote a hard sharing multi-task learning model (a function parameterized for instance, as a deep neural network) with parameters $\theta=\{\theta_{s}, \theta_{1}, \cdots, \theta_{T}\}$, that is trained to predict labels $\by_{\tau}$ of task $\tau$ from given samples $\bx_{\tau}$ as $\by_{\tau}=f_{\theta}(\bx_{\tau})$. Here, $\theta_{s}$ is the parameters shared across tasks and $\theta_{\tau}$ is the task specific parameters for task $\tau$ to predict the label based on the output from $\theta_{s}$. In multi-task learning, one commonly used criterion of learning $f_{\theta}$ is to minimize the following loss:
\begin{equation}\label{eq:multitask}
\mathcal{L}=\frac{1}{T}\sum_{\tau=1}^{T}\frac{1}{N_{\tau}}\sum_{\bx_{\tau}\in D_{\tau}}\ell_{\tau}(f_{\theta}(\bx_{\tau}),\by_{\tau}),
\end{equation}
where $\ell_{\tau}$ is the loss fuction (\eg Cross-Entropy loss function for classification) for task $\tau$.

\begin{figure}[h]
	\centering
	% include first image
	\includegraphics[width=.65\linewidth]{./figures/learning.pdf}  
	\vspace{-.2cm}
	\caption{Illustration of the learning process for both task 1 and task 2 using single task training, multi-task training and our method. Best seen in color.}
	\label{fig:learning}
	\vspace{-.1cm}
\end{figure}

\subsection{Knowledge Distillation for Multi-task Learning}
However, simply optimizing \cref{eq:multitask} may lead to worse overall performance due to the loss (task) imbalance \cite{sener2018multi,kendall2018multi,chen2017gradnorm} where some tasks' losses may dominate during optimization. Instead of developping a weigting scheme to assign dynamic weight to different tasks' losses, we consider optimizing the multi-task learning model using the idea of knowledge distillation. In another word, we aim at compressing the knowledge of the model that individually learns for each specific task into a single model. 

% To this end, we first train a single model $f_{\hat{\theta}_{\tau}}$ on each task $\tau$, where $\hat{\theta}_{\tau}=\{\theta_{s}, \theta_{\tau}\}$ and 
To this end, we first train a single model on each task $\tau$ and obtain the optimal model $f_{{\hat{\theta}_{\tau}}^{\star}}$ with parameters $\hat{\theta}^{\star}_{\tau}=\{{\theta^{\tau}_{s}}^{\star}, \theta^{\star}_{\tau}\}$.  We then use the single model $f_{{\hat{\theta}_{\tau}}^{\star}}$ to teach the multi-task model $f_{\theta}$:
\begin{equation}\label{eq:KDMT}
\mathcal{L}(\theta)=\frac{1}{T}\sum_{\tau=1}^{T}\left(\frac{\lambda}{N_{\tau}}\sum_{\bx_{\tau}\in D_{\tau}}\ell^{m}(\mathcal{A}_{\tau}(f_{\theta_s}(\bx_{\tau})), f_{{\theta^{\tau}_{s}}^{\star}}(\bx_{\tau}))+\frac{1}{N_{\tau}}\sum_{\bx_{\tau}\in D_{\tau}}\ell_{\tau}(f_{\theta}(\bx_{\tau}),\by_{\tau}) \right),
\end{equation}
where the function $\mathcal{A}_{\tau}:\mathbb{R}^{C\times H\times W}\rightarrow\mathbb{R}^{C\times H\times W}$ is a small adaptor for task $\tau$ to transform the intermediate feature (operate on $C$ dimension only) of the shared module in multi-task model $f_{\theta}$. $\ell^{m}()$ is the loss function to teach the multi-task model to produce similar features with the single model $f_{{\hat{\theta}_{\tau}}^{\star}}$ of task $\tau$ by:
\begin{equation}
\ell^{m}(\mathcal{A}_{\tau}(f_{\theta_s}(\bx_{\tau})), f_{{\theta^{\tau}_{s}}^{\star}}(\bx_{\tau}))=\left\lVert\frac{\mathcal{A}_{\tau}(f_{\theta_s}(\bx_{\tau}))}{||\mathcal{A}_{\tau}(f_{\theta_s}(\bx_{\tau}))||_2}-\frac{f_{{\theta^{\tau}_{s}}^{\star}}(\bx_{\tau})}{||f_{{\theta^{\tau}_{s}}^{\star}}(\bx_{\tau})||_2}\right\lVert_2^2.
\end{equation}



